Revealing the Chemical Structure of the Magellanic Clouds with APOGEE. I. Calculating Individual Stellar Ages of RGB Stars in the Large Magellanic Cloud

Stellar ages are critical for understanding the temporal evolution of a galaxy. We calculate the ages of over 6000 red giant branch stars in the Large Magellanic Cloud (LMC) observed with SDSS-IV / APOGEE-S. Ages are derived using multi-band photometry, spectroscopic parameters (T$_\text{eff}$, $\log{g}$, [Fe/H], and [$\alpha$/Fe]) and stellar isochrones and the assumption that the stars lie in a thin inclined plane to get accurate distances. The isochrone age and extinction are varied until a best match is found for the observed photometry. We perform validation using the APOKASC sample, which has asteroseismic masses and accurate ages, and find that our uncertainties are $\sim$20% and range from $\sim$1$-$3 Gyr for the calculated age values. Here we present the LMC age map as well as the age-radius relation and an accurate age-metallicity relation (AMR). The age map and age-radius relation reveal that recent star formation in the galaxy was more centrally located and that there is a slight dichotomy between the north and south with the northern fields being slightly younger. The northern fields that cover a known spiral arm have median ages of $\gtrsim$ 2 Gyr, which is the time when an interaction with the SMC is suggested to have happened. The AMR is mostly flat especially for older ages although recently (about 2.0-2.5 Gyr ago) there is an increase in the median [Fe/H]. Based on the time frame, this might also be attributed to the close interaction between the LMC and SMC.

==> authors.tex <==
% \author{APOGEE team}
% \affiliation{Department of Astronomy, University of Virginia, Charlottesville, VA, 22904, USA}

% \correspondingauthor{Joshua T. Povick}
% \email{joshua.povick@montana.edu}

\author[0000-0002-6553-7082]{Joshua T. Povick,$^{1}$,\thanks{joshua.povick@montana.edu}}
$^1$Department of Physics, Montana State University, P.O. Box 173840, Bozeman, MT 59717-3840
% \affiliation{Department of Physics, Montana State University, P.O. Box 173840, Bozeman, MT 59717-3840}

% \author[0000-0002-1793-3689]{David L. Nidever}
% \affiliation{Department of Physics, Montana State University, P.O. Box 173840, Bozeman, MT 59717-3840}
% \affiliation{National Optical Astronomy Observatory, 950 North Cherry Ave, Tucson, AZ 85719}

% \author[0000-0002-4818-7885]{Jamie Tayar}
% \affiliation{Florida}

% \author{Sten Hasselquist}
% \affiliation{Department of Physics \& Astronomy, University of Utah, Salt Lake City, UT 84112}

% \author[K. T. Smith et al.]{
% Keith T. Smith,$^{1}$\thanks{E-mail: publications@ras.ac.uk (KTS)}
% A. N. Other,$^{2}$
% Third Author$^{2,3}$
% and Fourth Author$^{3}$
% \\
% % List of institutions
% $^{1}$Royal Astronomical Society, Burlington House, Piccadilly, London W1J 0BQ, UK\\
% $^{2}$Department, Institution, Street Address, City Postal Code, Country\\
% $^{3}$Another Department, Different Institution, Street Address, City Postal Code, Country
% }

==> notes.tex <==
- change K band to Ks

- {\rm} 
